Correct Reasoning Paths Visit Shared Decision Pivots

Chain-of-thought (CoT) reasoning exposes the intermediate thinking process of large language models (LLMs), yet verifying those traces at scale remains unsolved. In response, we introduce the idea of decision pivots-minimal, verifiable checkpoints that any correct reasoning path must visit. We hypothesize that correct reasoning, though stylistically diverse, converge on the same pivot set, while incorrect ones violate at least one pivot. Leveraging this property, we propose a self-training pipeline that (i) samples diverse reasoning paths and mines shared decision pivots, (ii) compresses each trace into pivot-focused short-path reasoning using an auxiliary verifier, and (iii) post-trains the model using its self-generated outputs. The proposed method aligns reasoning without ground truth reasoning data or external metrics. Experiments on standard benchmarks such as LogiQA, MedQA, and MATH500 show the effectiveness of our method.

==> algorithm.tex <==
\setlength{\algomargin}{1.6em}
\SetNlSty{textbf}{}{.}
\SetNlSkip{0.4em}
\SetAlgoNlRelativeSize{0}

\begin{algorithm}[H]
\caption{Reasoning Optimization via Multi-path Aggregation}
\label{alg:roma}\footnotesize
\textbf{Inputs:} $p_{\theta}$ (reasoner), $v_{\psi}$ (verifier; LoRA on $p_{\theta}$), dataset $\mathcal{D}$, samples $K$, rounds $L$, DPO temp. $\beta$, batch size $B$\\
\textbf{Output:} Updated parameters $\theta$
\BlankLine

$p_{\rm ref}\leftarrow\texttt{StopGradient}(p_{\theta})$ \tcp*{Frozen DPO reference}
\For{$\ell\gets1$ \KwTo $L$}{
  $\mathcal{P}\leftarrow\varnothing$ \;
  \ForEach{$(x_i,y_i)\in\mathcal{D}$}{
    \tcp{A: sample and filter candidates using \cref{eq:sets}; stop when $K$ paths collected}
    $\mathcal{S}_i\leftarrow\varnothing,\; R_i^{+}\leftarrow\varnothing$\;
    \While{$|\mathcal{S}_i|<K$}{
      draw $r\sim p_{\theta}(r\mid x_i)$ \tcp*{per \cref{eq:sets}}
      $\mathcal{S}_i\leftarrow \mathcal{S}_i\cup\{r\}$\;
      \If{$\arg\max_{y} p_{\theta}(y\mid x_i,r)=y_i$}{$R_i^{+}\leftarrow R_i^{+}\cup\{r\}$}
    }
    \If{$|R_i^{+}|=0$}{\textbf{continue}}
    \tcp{B: synthesize short path (\cref{eq:verifier})}
    $\hat r_i\leftarrow v_{\psi}(x_i,R_i^{+})$;\;
    \If{$\arg\max_y p_{\theta}(y\mid x_i,\hat r_i)\neq y_i$}{
      $\hat r_i\leftarrow\arg\max_{r\in R_i^{+}} p_{\theta}(y_i\mid x_i,r)$
    }
    \tcp{C: build preferences (\cref{eq:prefset})}
    $\mathcal{P}\leftarrow\mathcal{P}\cup\{(\hat r_i,r): r\in R_i^{+}\setminus\{\hat r_i\}\}$\;
  }
  \ForEach{\textnormal{minibatch } $\mathcal{B}\subset\mathcal{P}$ \textnormal{ of size } $B$}{
    Update $\theta$ with $\mathcal{L}_{\mathrm{DPO}}(\theta;\mathcal{B},p_{\rm ref},\beta)$ \textnormal{using} \cref{eq:dpo}\;
  }
}
\Return $\theta$
\end{algorithm}


==> tab/logiqa.tex <==
\begin{tabular}{l c}
\toprule
\textbf{Method} & \textbf{Overall Acc.} \\
\midrule
Zero-Shot & 0.420 \\
%\multicolumn{2}{c}{\textbf{Zero-Shot}}\\
%\midrule
%\quad 0.6B & 0.42 \\
%\quad 1.7B & 0.64 \\
%\quad 4B   & 0.72 \\
%\quad 8B   & 0.74 \\
%\quad 14B  & 0.86 \\
\midrule
\multicolumn{2}{c}{\textbf{Trained without Reasoning}}\\
\midrule
\quad SFT & 0.412 ($\downarrow0.008$)\\
\midrule
\multicolumn{2}{c}{\textbf{Self-Trained with Zero-Shot Reasoning}}\\
\midrule
\quad SFT & 0.395 ($\downarrow0.025$)\\
\midrule
\multicolumn{2}{c}{\textbf{Self-Trained with Max ROSCOE Reasoning}}\\
\midrule
\quad SFT      & 0.446 ($\uparrow0.026$)\\
\quad SFT+DPO  & 0.477 ($\uparrow0.057$)\\
\midrule
\multicolumn{2}{c}{\textbf{Self-Trained with Short-Path Reasoning w/o. verifier}}\\
\midrule
\quad SFT      & 0.462 ($\uparrow0.042$) \\
\quad SFT+DPO  & \textbf{0.495} ($\uparrow0.083$) \\
\quad DPO  & \textbf{0.489} ($\uparrow0.077$) \\
\midrule
\multicolumn{2}{c}{\textbf{Self-Trained with Short-Path Reasoning (Ours) }}\\
\midrule
\quad DPO  & \textbf{0.518} ($\uparrow0.098$) \\
\bottomrule
\end{tabular}

%495 - 0412

==> tab/math500.tex <==
\begin{tabular}{l c}
\toprule
\textbf{Method} & \textbf{Overall Acc.} \\
\midrule
Zero-Shot & 0.636 \\
%\multicolumn{2}{c}{\textbf{Zero-Shot}}\\
%\midrule
%\quad 0.6B & 0.42 \\
%\quad 1.7B & 0.64 \\
%\quad 4B   & 0.72 \\
%\quad 8B   & 0.74 \\
%\quad 14B  & 0.86 \\
\midrule
\multicolumn{2}{c}{\textbf{Trained without Reasoning}}\\
\midrule
\quad SFT &  0.649 ($\uparrow0.013$)\\
\midrule
\multicolumn{2}{c}{\textbf{Self-Trained with Zero-Shot Reasoning}}\\
\midrule
\quad SFT &  0.655 ($\uparrow0.019$)\\
\midrule
\multicolumn{2}{c}{\textbf{Self-Trained with Max ROSCOE Reasoning}}\\
\midrule
\quad SFT      &  0.673($\uparrow0.037$)\\
\quad SFT+DPO  &  0.681($\uparrow0.045$)\\
\midrule
\multicolumn{2}{c}{\textbf{Self-Trained with Short-Path Reasoning w/o. verifier}}\\
\midrule
\quad SFT      &  0.669 ($\uparrow0.033$) \\
\quad SFT+DPO  & \textbf{0.684} ($\uparrow0.048$) \\
\quad DPO  & \textbf{0.681} ($\uparrow0.045$) \\
\midrule
\multicolumn{2}{c}{\textbf{Self-Trained with Short-Path Reasoning (Ours) }}\\
\midrule
\quad DPO  & \textbf{0.702} ($\uparrow0.066$) \\
\bottomrule
\end{tabular}


==> tab/medqa.tex <==
\begin{tabular}{l c}
\toprule
\textbf{Method} & \textbf{Overall Acc.} \\
\midrule
Zero-Shot & 0.159 \\
\midrule
\multicolumn{2}{c}{\textbf{Trained without Reasoning}}\\
\midrule
\quad SFT & 0.204 ($\uparrow0.045$)\\
\midrule
\multicolumn{2}{c}{\textbf{Self-Trained with Zero-Shot Reasoning}}\\
\midrule
\quad SFT & 0.215 ($\uparrow0.056$)\\
\midrule
\multicolumn{2}{c}{\textbf{Self-Trained with Max ROSCOE Reasoning}}\\
\midrule
\quad SFT      & 0.232 ($\uparrow0.073$)\\
\quad SFT+DPO  & 0.239 ($\uparrow0.080$)\\
\midrule
\multicolumn{2}{c}{\textbf{Self-Trained with Short-Path Reasoning w/o. verifier}}\\
\midrule
\quad SFT      & 0.234 ($\uparrow0.075$) \\
\quad SFT+DPO  & \textbf{0.251} ($\uparrow0.092$) \\
\quad DPO  & \textbf{0.250} ($\uparrow0.091$) \\
\midrule
\multicolumn{2}{c}{\textbf{Self-Trained with Short-Path Reasoning (Ours) }}\\
\midrule
\quad DPO  & \textbf{0.316} ($\uparrow0.157$) \\
\bottomrule
\end{tabular}

%495 - 0412
